Beyond Image Super-Resolution for Image Recognition with Task-Driven Perceptual Loss

In real-world scenarios, image recognition tasks, such as semantic segmentation and object detection, often pose greater challenges due to the lack of information available within low-resolution (LR) content. Image super-resolution (SR) is one of the promising solutions for addressing the challenges. However, due to the ill-posed property of SR, it is challenging for typical SR methods to restore task-relevant high-frequency contents, which may dilute the advantage of utilizing the SR method. Therefore, in this paper, we propose Super-Resolution for Image Recognition (SR4IR) that effectively guides the generation of SR images beneficial to achieving satisfactory image recognition performance when processing LR images. The critical component of our SR4IR is the task-driven perceptual (TDP) loss that enables the SR network to acquire task-specific knowledge from a network tailored for a specific task. Moreover, we propose a cross-quality patch mix and an alternate training framework that significantly enhances the efficacy of the TDP loss by addressing potential problems when employing the TDP loss. Through extensive experiments, we demonstrate that our SR4IR achieves outstanding task performance by generating SR images useful for a specific image recognition task, including semantic segmentation, object detection, and image classification. The implementation code is available at https://github.com/JaehaKim97/SR4IR.

==> sections/submission/7_archives.tex <==
%%%%%%%%% Introduction_v0.tex %%%%%%%%%%
\section{Introduction}
\label{sec:introduction}
%
Single image super-resolution~(SR) is a fundamental computer vision problem, which aims to restore high-resolution~(HR) images from given low-resolution~(LR) images.
% 
% Since SR is a kind of image processing that increases the image resolution, we can apply SR as pre-processing for various computer vision tasks.
SR is also known as low-level vision, which means that it can be used as a pre-processing for various scenarios.
% 

After pioneering AlexNet~\cite{cls_alexnet}, numerous deep neural network-based methods achieve superior performance in various computer vision tasks, such as image classification~\cite{cls_resnet, cls_conv2020s, net_densenet, cls_effnet, net_mobilenet, net_vgg, misc_vit}, object detection~\cite{det_fasterrcnn, det_retinanet, det_ssd, det_yolo}, and semantic segmentation~\cite{seg_deeplab, seg_fcn, zhang2022topformer, xie2021segformer}.
% 
% These methods directly take images as input for the neural network, which we denote as \textit{task} network in this paper.
% These methods are often trained in an end-to-end manner, which means the network directly takes images as input and then outputs the task results, which we denote the network as \textit{task} network in this paper.
These approaches begin by feeding images as input to a neural network, then generate task-specific results, \eg, predicted label in image classification, by extracting and processing information from the images using a deep neural network, which we refer to \textit{task} network in this paper.
%

% When the input images are LR, the performance of the task network is significantly degraded, as input images lose the amount of high-frequency parts, which can be key features for performing the task.
However, in practical scenarios, input images are often subject to degradation into LR versions due to various factors, including camera limitations or data transformations.
% 
When the input images are in a LR, the performance of the task network experiences a significant decline.
% 
This degradation occurs because LR images lack crucial high-frequency components, which often contain features necessary for executing the task.
% 
In this case, employing SR as a pre-processing step emerges as a promising solution~\cite{sr_tdsr, zhou2021improving}, as SR is renowned for its ability to restore high-frequency details.
% 
In these scenarios, the primary role of SR lies in its ability to restore high-frequency regions that encompass essential task-related features.
% 
Throughout this paper, our objective is to introduce a \textit{unified} SR framework combined with a task network.
%
This involves the joint training of both the SR and task networks, with a focus on emphasizing the task-related benefits while concurrently achieving photo-realistic SR results.
% 


% 
% Through this paper, our objective is to illustrate the training of the SR network with an emphasis on task-related benefits, all while generating photo-realistic SR outcomes.
% 
% In other words, the restoration of high-frequency regions, which contain crucial task-related features, becomes paramount in such cases.
% 

% In this case, applying SR as a pre-process is one of the promising solutions, as SR is known to restore high-frequency parts, \ie, resulting in a high peak signal noise ratio~(PSNR).
% % 
% However, an input image with a higher PSNR does not always guarantee surpassing task performance for the given task network.
% % 
% For example, consider the case of performing image classification on an LR image with dog class.
% %
% Even with a low PSNR of the background, an image including an apparent dog is still a good image for the perspective of the task network.
% % 
% In other words, the SR network that is optimized on the PSNR is sub-optimal for the task perspective, and we need to let the SR network take more focus on where the task network sees as meaningful.
% 

The conventional SR literature~\cite{sr_edsr, sr_swinir, sr_rdn, sr_vdsr, sr_dbpn, rs_ircnn} has predominantly centered on image restoration by minimizing pixel-wise errors between HR and SR results, with the primary aim of achieving high PSNR (Peak Signal-to-Noise Ratio) values.
% 
However, the pursuit of higher PSNR values does not inherently guarantee the restoration of informative high-frequency details that are essential for the task at hand.
% 
For instance, in the context of image classification, if a high PSNR achievement is attributed to well-restored background regions, such processing does not guarantee an enhancement in task performance, as the critical factor lies in restoring high-frequency areas containing the object itself.
% 
To address the challenge, rather than concentrating on minimizing pixel-wise errors within the image space, we focus on errors within the feature space, commonly referred to as perceptual loss~\cite{misc_perceptual}.
% 
% Then, how can we effectively train the SR network to prioritize the restoration of high-frequency regions that are essential for task perspective?
% To address this challenge, we explore effective ways to train the SR network to prioritize the restoration of high-frequency regions essential from a task perspective, all the while ensuring the generation of visually pleasing SR results.
% 
% Incorporating perceptual loss~\cite{misc_perceptual} is a well-established technique in SR that aims to restore photo-realistic results.
% 

% When input images are fed into the task network, the deep neural network processes the image features in a manner that aids in task execution~\cite{}.
% Hence, computing the perceptual loss within the feature space of the task network can directly instruct the SR network to restore high-frequency regions relevant to the task.
The conventional perceptual loss is computed by measuring the distance between the SR and HR images in the deep feature space, such as VGG~\cite{net_vgg} features pre-trained on ImageNet~\cite{data_imagenet}.
% 
However, when we compute the perceptual loss within the feature space of the task network, it acquires greater relevance from a task-oriented perspective.
% 
When input images are fed into the task network, the deep neural network manipulates image features in a manner that enhances task execution.
% 
Hence, by computing the perceptual loss within the feature space of the task network, we can directly guide the SR network to restore high-frequency regions that are pertinent to the task, a concept we refer to as Task-Driven Perceptual~(TDP) Loss.
% 

As our TDP loss is computed within the feature space of the task network, its behavior is significantly influenced by the knowledge and features that the task network acquires.
% 
In simpler terms, the way we train the task network is a crucial factor in defining how the TDP loss operates.
% 
However, it's worth noting that if the task network is trained to rely on specific features, such as shortcut learning~\cite{geirhos2020shortcut}, the effectiveness of TDP may diminish, as it can potentially constrain the SR to restore other essential features.
% 
To overcome this challenge, we propose a novel training strategy called Cross-Quality Patch Mix~(CQMix), which trains the task network using not only HR or SR images but also patch-wise mixed versions of HR and SR images.
% 
By employing this strategy, the task network learns to utilize various features, allowing us to fully harness the capabilities of TDP.
%


Nonetheless, when both the SR and task networks are trained simultaneously, simply incorporating the TDP loss can lead to unintended local minima.
% 
This occurs because, when the task network is trainable, the TDP loss forces the task network to generate the same features when processing both HR and SR images, rather than encouraging updates to the SR network for the restoration of high-frequency details.
% 
Therefore, we introduce an alternate training framework, which sequentially updates the SR network and task networks at each iteration, enabling the TDP loss to entirely focus on restoring the task-relevant high-frequency part.
% 
% As a result, by combining the proposed TDP, CQMix, and alternate training framework, we substan


In this paper, we have examined the integration of SR with three representative computer vision tasks: image classification, semantic segmentation, and object detection.
% 
Our extensive experiments demonstrate that the proposed framework significantly improves the performance compared to the baseline, which is trained only on LR images or uses intuitive SR combined methods.
% 
These results indicate that our framework can be adopted in a wide range of applications.
% 
As high-level vision task combined with SR problem is barely studied, we hope our work could provide useful insights into the following works.
% 
We summarize our contributions as follows:

\input{figs/submission/1/overview/main_figure}

%%%%%%%%% proposed_method_copy.tex %%%%%%%%%%
\section{Proposed method}
\label{sec:proposed_method}
%
\paragraph{Notation.}
Let $\boldsymbol{I}_\text{HR} \in \mathbb{I}_\text{HR}$ and $\boldsymbol{I}_\text{LR} \in \mathbb{I}_\text{LR}$ denote the high-resolution (HR) and low-resolution (LR) images, paired with their corresponding task labels $\boldsymbol{y} \in \mathbb{Y}$ (\eg, class labels in image classification task).
$f_{\boldsymbol{\theta}_{\text{SR}}}: \mathbb{I}_\text{LR} \rightarrow \mathbb{I}_\text{SR}$ denotes the super-resolution (SR) network parameterized by $\boldsymbol{\theta}_{\text{SR}}$ where $\mathbb{I}_\text{SR}$ is the super-resolved image set.
Given the SR or HR images, we predict corresponding labels using the task network parameterized by $\boldsymbol{\theta}_{\text{Task}}$: $f_{\boldsymbol{\theta}_{\text{Task}}}: \mathbb{I}_\text{SR} \cup \mathbb{I}_\text{HR} \rightarrow \mathbb{Y}$.

\paragraph{Problem Definition.}
The goal of task-aware super-resolution is to produce photo-realistic images from $\boldsymbol{I}_\text{LR}$ that can benefit the subsequent high-level vision task, which is formally given by
\begin{equation}\label{eq:problem_definition}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{SR}},\boldsymbol{\theta}_{\text{Task}}} & \mathcal{L}_{\text{SR}}(f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{I}_\text{HR}) \\ & + \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} \circ f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{y}),
    \end{aligned}
\end{equation}
where the first and second term is for evaluating the quality of the super-resolved results and the performance for the target high-level vision task, respectively.



% task relevant knowledge를 이용하여 sr학습하는게 성능에 도움이 되는가?
% 그렇다면 어떻게 transmit해야하나?
%-> 우리는 sec 3.2에서 task-driven perceptual loss + cyclic training 을 통해 task-relevant feature를 이용해 sr을 할습시킬 수 있음을 보인다
% 3.3에서는 더 효과적인 transmission을 위해선 task net을 어떻게 학습시키는지도 중요...


\iffalse
To this end, we define the objective of task-aware super-resolution training as follows:
\begin{equation}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{SR}},\boldsymbol{\theta}_{\text{Task}}} & \mathcal{L}_{\text{SR}}(\boldsymbol{I}_\text{SR},\boldsymbol{I}_\text{HR},\boldsymbol{y},f_{\boldsymbol{\theta}_{\text{Task}}}) \\ & +\mathcal{L}_{\text{Task}}(\boldsymbol{I}_\text{SR},\boldsymbol{I}_\text{HR},\boldsymbol{y},f_{\boldsymbol{\theta}_{\text{Task}}}),
    \end{aligned}
\end{equation}
where $f_{\boldsymbol{\theta}_{\text{SR}}}$ and $f_{\boldsymbol{\theta}_{\text{Task}}}$ indicate the SR and task network parameterized by $\boldsymbol{\theta}_{\text{SR}}$ and $\boldsymbol{\theta}_{\text{Task}}$, respectively, and $\boldsymbol{I}_\text{SR}=f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR})$.
The first term for training the SR network incorporates task-relevant losses in addition to the standard losses for SR training to encourage the SR network to produce images that are advantageous for subsequent high-level vision tasks.
The second term for training the task network is designed not only to enhance the ability to process SR images for improved performance but also to learn task-specific knowledge that can be effectively transmitted to the SR network.
\fi

% 수식: l_sr, l_task -> 각 각의 의미 설명하면서 이 논문의 목표 설명

% s+t 구조 설명 (l1, celoss)

% sr net이 task-relavant 정보를 학습하기 위해서는 ce loss로는 부족. perceptual loss를 쓰자
% 그런데 s+t 구조에서는 쓰기 어려움
% 따라서 우리는 cyclic한 구조 제안 -> cycle 1,2의 의미 설명

% cycle 2에서 task net을 어떻게 학습하냐가 중요
% hr, sr, mix ...

\iffalse
%
Given HR and LR images, denoted as $x_\text{HR}$ and $x_\text{LR}$, along with their corresponding target task label $y$ (\eg, image label in classification), our objective is to reconstruct $x_\text{SR}$ from $x_\text{LR}$ in a manner that benefits the prediction of the task label $y$, while simultaneously achieving visually realistic super-resolution results.
% 
With mathematical formulation, for the SR network~$\mathbf{S}$ and the task network~$\mathbf{T}$, the objective term can be defined as follows:
% 
\begin{equation}
    \begin{split}
            % x_\text{SR} =\; &\mathbf{S}\paren{x_\text{LR}}, \\
            % \text{miminize} \;\;\; &\text{LPIPS} \paren{x_\text{SR}, x_\text{HR}}, \\
            % \text{miminize} \;\;\; &\mathcal{L}_\text{task}\paren{\mathbf{T}\paren{x_\text{SR}}, y}, \\
            x_\text{SR} =\; \mathbf{S}\paren{x_\text{LR}}, \\
            \textit{miminize} \;\;\; \mathcal{L}_\text{LPIPS} \paren{x_\text{SR}, x_\text{HR}}, \\
            \textit{minimize} \;\;\; \mathcal{L}_\text{task}\paren{\mathbf{T}\paren{x_\text{SR}}, y}, \\
    \end{split}
    \label{eq:notation}
\end{equation}
% 
where LPIPS~\cite{zhang2018perceptual} is image perceptual quality measurement with lower is better, and Task-Metric stands for metrics for corresponding tasks, \eg, top-1 accuracy in classification.
% 
\fi

\subsection{Overview: Cyclic Training}
\iffalse
In the following subsections, we elaborate on the proposed method by exploring our motivational question: \textit{how to effectively transfer task-relevant knowledge to SR network?}
In Section~\ref{subsec:percep}, we propose task-driven perceptual loss with cyclic training to encourage the SR network to learn task-relevant knowledge, thereby enhancing the performance of the following task.
In Section~\ref{subsec:mixup}, based on our observation that training a task network using only HR images deteriorates the performance, we introduce a novel cross-quality patch mix-up strategy.
We demonstrate that this strategy encourages the task network to acquire more transferable knowledge for the SR network.
The overview of the proposed method is illustrated in Figure~\ref{fig:main_figure}.
\fi

% tasr의 목표를 달성하기 위해선 우리는 다음과 같은 질문에 답해야한다
% "sr network가 어떻게 task network로 부터 task 정보를 학습해야하는가"
% "task network가 어떻게 효과적으로 sr network에게 정보를 전달 해줄 수 있는가"

To achieve the goal of task-aware super-resolution, a key question arises: \textit{How can we leverage the HR images and the task network to prompt the SR network to learn task-specific knowledge?}
Our strategy to address this question involves a cyclic training framework, alternating the training between the SR and task networks.
Figure~\ref{} illustrates the overview of our cyclic training scheme.
In the first cycle, the SR network is trained to generate images beneficial for the task network.
In the second cycle, the task network learns task-specific knowledge that will be transferred to the SR network in the subsequent cycle.
We elaborate on the details of the cyclic training framework in the following subsections.
In section~\ref{subsec:percep}, we introduce task-driven perceptual loss in the first cycle to encourage the SR network to imitate the task-relevant features present in HR images.
In section~\ref{subsec:mixup}, we share our observation that a task network trained solely on HR images learns less transferable features for the SR network.
Based on the observation, we introduce Cross-Quality patch Mix technique in the second cycle that prevents the task network from focusing on shortcuts, thereby enhancing the transferability for the SR network.


\subsection{Cycle 1: Task-Driven Perceptual Loss}\label{subsec:percep}
Owing to the abundance of features within HR images, training the task network with HR images achieves substantially better task performance compared to training with LR images.
For task-aware super-resolution to succeed, the SR network should strive to emulate HR images, particularly focusing on incorporating the task-relevant features present in HR images.
To this end, inspired by the concept of perceptual loss~\cite{leon2015_texture,misc_perceptual}, we propose task-driven perceptual loss that promotes the generation of SR images that imitate task-relevant and perceptually pleasing features within the HR images learned by the task network.
Formally, we define the task-driven perceptual loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{percep}} = \frac{1}{B} \sum_{i=1}^{B} \lVert f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
where $B$ is the batch size and the superscript in each image notation indicates the index of images in a batch.


In cycle 1, we train the SR network using the task-driven perceptual loss and the reconstruction loss between SR and HR images:
\begin{equation}
    \mathcal{L}_{\text{cycle 1}} = \mathcal{L}_{\text{percep}} + \mathcal{L}_{\text{recon}},
\end{equation}
where $\mathcal{L}_{\text{recon}} = \frac{1}{B} \sum_{i=1}^{B} \lVert \boldsymbol{I}_\text{SR}^i - \boldsymbol{I}_\text{HR}^i \rVert_1$.



\subsection{Cycle 2: Cross-Quality Patch Mix}\label{subsec:mixup}
To enhance the effectiveness of the task-driven perceptual loss, it is crucial that the task network learns task-specific features embedded in the HR images in cycle 2.
An intuitive approach is to train the task network with HR images.
Yet, we observe that training solely with HR images offers limited performance gain from the task-driven perceptual loss.
Instead, we find that training the task network using both the HR and upscaled LR images produces more performance gain.
Our hypothesis regarding this phenomenon is that training solely with HR images leads to shortcut learning, utilizing only a subset of HR image features for training.
This, in turn, hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
Figure~\ref{} illustrates the conceptual description of our hypothesis.
For a detailed analysis of these observations, please refer to Section~\ref{}.

Based on our observation, we propose a novel data augmentation strategy called \textbf{C}ross-\textbf{Q}uality patch \textbf{Mix} (CQMix) that further enhances the efficacy of the task-driven perceptual loss by encouraging the task network to learn more transferable knowledge for the SR network.
CQMix augments an image by randomly choosing either HR or SR patches within each grid region.
By doing so, CQMix creates an image where high-frequency components are randomly erased, effectively preventing the task network from learning shortcuts that are not transferable to the SR network.
Figure~\ref{} illustrates CQMix method and its intuitive meanings.
% 그래서 task net이 hr의 특정 feature에만 집중해서 학습하는걸 막고 다양한 feature를 학습하도록 강제함
%

\iffalse
\subsection{Cyclic Training}
Conventionally, the perceptual loss is calculated using pretrained and fixed network.
In the context of task-aware super-resolution, implementing the task-driven perceptual loss becomes difficult since it is essential to train the task network for the target task.
There are several possible approaches: pretraining the task network and keeping it fixed during training of the SR network or utilizing the pretrained network as an additional network solely for calculating the perceptual loss.
However, we find that the performance gain of the task-driven perceptual loss in these strategies is marginal.
We attribute the phenomenon to (?).
% cyclic -> 
To resolve these issues, we propose a cyclic training framework where the task and SR network are alternatively trained.
In the first cycle, we train only the task network using a task-specific loss (\eg, cross-entropy loss) with SR or HR images.
The subsequent cycle then trains the SR network with the fixed task network using $\ell_1$ loss between HR and SR images, GAN loss~\cite{}, and the task-driven perceptual loss.
We observe that the cyclic training scheme boosts the performance gain from the task-driven perceptual loss since (?).
\fi


% percep loss는 원래 있잖아?
% 우리가 다른점: target task를 위한 network에 percep loss + cyclic training으로 task net도 점진적으로 학습 + sr net도 점진적으로 받아들임
% 강조할 수 있는 방법: 첫번째 차이점은 적당히 강조. 너무 강조하면 역효과. 두번째는 "pretrained fixed network를 사용할 경우 sr이 이로부터 학습하는것이 어려울것임.

% HR image는 task 입장에서 활용할 정보가 많아서 (eg. detailed texture, shape...) task 성능을 좋게함
% 이러한 task-specific 정보는 task net intermediate feature에 존재 (cite)
% tasr의 목표를 달성하기 위해선, task network 입장에서 sr과 hr을 identically perceive 하도록 해야함
% 따라서 우리는 hr에 담긴 task-relevant 정보를 학습하면서도 sr quality를 높이기 위한 방법으로 task-driven perceptual loss를 사용하는 것을 제안(cite), 수식
% task-driven loss는 sr을 task에 필요한 high-level feature를 살리기 때문에 visually pleasing하면서 task에 도움이 되는 sr 이미지 생성할 수 있도록 도와줌

% conventionally pretrained fixed network 사용함
% 하지만 우리는 이렇게 percep loss를 사용할 경우 percep으로 인한 gain이 미미함을 관찰
% 우리는 이러한 이유를 training 초기에 sr과 hr의 feature 상에서의 gap이 너무 크기 때문이라고 생각 (?)
% 이를 해결하기 위해 우리는 점진적으로 학습되는 task network로 부터 guide를 받을 수 있는 cyclic framework을 제안
% cycle 1: task network가 task 정보를 학습하는 단계
% cycle 2: 학습된 task network로 부터 sr에 정보 전달하여 학습하는 단계


Consequently, we train the task network in cycle 2 using task-specific loss using SR, HR, and augmented images by CQMix:
\begin{equation}
    \min\limits_{\boldsymbol{\theta}_\text{Task}} \; \sum_{i=1}^B \mathcal{L}_{\text{task}}(f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}^i),\boldsymbol{y}),
\end{equation}


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/submission/3.1/overview5.pdf}
    \\
    \figspace
    \caption{
        %
        \textbf{Overview of the proposed TaSR.}
        % 
    }
    \label{fig:main_figure}
    \figxspace
\end{figure*}

%%%%%%%%% proposed_method_v0.tex %%%%%%%%%%


\section{Proposed method}
\label{sec:proposed_method}
%
% Training the task network on HR images can achieve significantly superior results compared to training on their LR counterparts.
% % 
% This distinction is because LR images lack essential high-frequency details, which often contain crucial task-related features.
% % 
% Therefore, to succeed in task-aware super-resolution, the SR network should prioritize restoring high-frequency regions, with a specific emphasis on the task-relevant features present in HR images.
% 
\paragraph{Notation.}
Let $\boldsymbol{I}_\text{HR} \in \mathbb{I}_\text{HR}$ and $\boldsymbol{I}_\text{LR} \in \mathbb{I}_\text{LR}$ denote the high-resolution (HR) and low-resolution (LR) images, paired with their corresponding task labels $\boldsymbol{y} \in \mathbb{Y}$ (\eg, class labels in image classification task).
$f_{\boldsymbol{\theta}_{\text{SR}}}: \mathbb{I}_\text{LR} \rightarrow \mathbb{I}_\text{SR}$ denotes the super-resolution (SR) network parameterized by $\boldsymbol{\theta}_{\text{SR}}$ where $\mathbb{I}_\text{SR}$ is the super-resolved image set.
Given the SR images~$\boldsymbol{I}_\text{SR}$, we predict corresponding labels using the task network parameterized by $\boldsymbol{\theta}_{\text{Task}}$: $f_{\boldsymbol{\theta}_{\text{Task}}}: \mathbb{I}_\text{SR} \rightarrow \mathbb{Y}$.

\paragraph{Problem Definition.}
The goal of task-aware super-resolution is to produce photo-realistic images from $\boldsymbol{I}_\text{LR}$ that can benefit the subsequent high-level vision task, which is formally given by
\begin{equation}\label{eq:problem_definition}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{SR}},\boldsymbol{\theta}_{\text{Task}}} & \mathcal{L}_{\text{SR}}(f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{I}_\text{HR}) \\ & + \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} \circ f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{y}),
    \end{aligned}
\end{equation}
where the first and second terms are used to evaluate the quality of the super-resolved results and the performance for the target high-level vision task, respectively.

\subsection{Task-Driven Perceptual Loss}\label{subsec:percep}
% mse < percep : sr 측면에서
% 우리는 percep loss를 sr quality를 높이는거 + task에 도움이 되는 feature 집중해서 살리기 위해서
%
\iffalse
High-resolution (HR) images contain abundant high-frequency details crucial for achieving superior performance in high-level vision tasks, compared to low-resolution (LR) images.
%The concept of perceptual loss~\cite{leon2015_texture,misc_perceptual} is proposed to restore the high-frequency contents of HR images by increasing the similarity between HR and SR images in a feature space of a fixed pre-trained network.
Perceptual loss~\cite{leon2015_texture,misc_perceptual} is a widely used technique in the SR field to restore the high-frequency components present in HR images.
Conventionally, the perceptual loss is often calculated within a feature space of VGG network pre-trained on ImageNet, which might be irrelevant to a target task.
In the context of the task-aware super-resolution problem, however, it is essential for the SR network to strive to emulate HR images, particularly focusing on features relevant to a target task.
% percep loss는 widely used technique for enhancing~
% conventionally, imagenet pre-trained
% In the context of tasr problem, however, we argue that task에 맞춰 학습된 network로 부터 percep loss 주는게 tasr의 performance를 위해 효과적
%For task-aware super-resolution to succeed, the SR network should strive to emulate HR images, particularly focusing on incorporating the task-relevant features present in HR images. 이게 위에 문장에 들어가기
To this end, we propose task-driven perceptual loss, a more flexible usage of perceptual loss, that is calculated using the network trained on a target task.
By doing so, our task-driven perceptual loss can promote the generation of SR images that imitate not just visually appealing but also task-relevant high-frequency details contained in the HR images.
Formally, we define the task-driven perceptual loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{percep}} = \frac{1}{B} \sum_{i=1}^{B} \lVert f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
where $B$ is the batch size, and the superscript in each image notation indicates the index of images in a batch.
\fi

Perceptual loss~\cite{leon2015_texture, misc_perceptual} is a widely adopted technique in the field of SR to restore the high-frequency components.
% 
As the perceptual loss quantifies the difference between SR and HR images in the feature space, the definition of this feature space significantly impacts the function of perceptual loss.
% 
Conventionally, the perceptual loss is computed within the feature space of a VGG network pre-trained on ImageNet.
% 
However, this feature space may not be directly relevant to the target task, and simply employing perceptual loss does not contribute to improving the performance of the subsequent task network $f_{\boldsymbol{\theta}_\text{Task}}$.
%


To this end, we propose task-driven perceptual~(TDP) loss, which offers a more flexible usage of perceptual loss by calculating the distance using the feature space of the task network, which is trained on a target task.
% 
When input images are fed into the task network, the deep neural network manipulates image features in a manner that enhances task execution.
% 
Hence, by computing the perceptual loss within the feature space of the task network, we can directly guide the SR network to restore high-frequency regions that are pertinent to the task.
% 
The TDP loss encourages the generation of SR images that not only appear visually appealing but also contain task-relevant high-frequency details.
% 
Formally, we define the TDP loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
% 
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{TDP}} = \frac{1}{B} \sum_{i=1}^{B} \lVert \phi_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - \phi_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
% 
where $B$ is the batch size, $\phi$ is an intermediate activation of the task network $f$, and the superscript in each image notation indicates the index of images in a batch.
% 


%In the following subsections, we introduce novel techniques to further enhance the effectiveness of our task-driven perceptual loss.
%In Section~\ref{subsec:mix}, we propose a novel data augmentation technique tailored for the task-aware super-resolution problem.
%In Section~\ref{subsec:alternate}, we propose an alternate training scheme that enables more gentle usage of the task-driven perceptual loss.


% 우리의 목표는 sr task 둘다 학습시키는 것
% 따라서 task network는 학습이 진행됨에 따라 계속 변함
% 이 상황에서 task percep을 줄 수 있는 방법은 additional pre-trained model 두는 것
% 하지만 이럴경우 
% 따라서 우리는 ~ 하기 위해 alterate training framework을 제안
% cycle 1 에서는~
% cycle 2 에서는~



\subsection{Cross-Quality Patch Mix}\label{subsec:mix}
\iffalse
The effectiveness of the task-driven perceptual loss is inherently related to the training procedure for the task network.
For high-level vision tasks, it is widely known that a network is susceptible to shortcut learning~\cite{geirhos2020shortcut}, which means a network relies on superficial and non-intrinsic features in training data, leading to poor generalization ability.
%cite classification suffer shortcut learning
% this could make the task-percep loss less effective since utilizing only a subset of HR image features hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
%We hypothesize that training solely with HR images leads to shortcut learning, utilizing only a subset of HR image features for training.
%This, in turn, hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
%Figure~\ref{} illustrates the conceptual description of our hypothesis.
Notably, shortcut learning can pose challenges in the problem of task-aware super-resolution, as the shortcut features learned by a task network can hinder the SR network from acquiring comprehensive features present in HR images through task-driven perceptual loss.
For instance, if a task network exclusively learns beak features to classify bird species, the task-driven perceptual loss may struggle to effectively guide the SR images to restore other key high-frequency contents, such as the feather and shape, limiting both the quality of SR results and the task performance.
Indeed, we observe that training the task network solely with HR images weakens the effectiveness of the task-driven perceptual loss, which is analyzed in Section~\ref{}.
\fi

Since our TDP loss operates within the feature space of the task network, its effectiveness is inherently linked to the training process of the task network.
% 
One possible approach is to utilize the feature space of a frozen task network pre-trained on HR images, similar to the conventional perceptual loss.
% 
However, it's crucial to recognize that task networks are susceptible to shortcut learning~\cite{geirhos2020shortcut}, a phenomenon where a network relies on superficial and non-intrinsic features in the training data.
% 
Notably, when we use a TDP loss using the task network trained with such shortcut learning, it can pose challenges, as it may hinder the SR network from acquiring the comprehensive features present in HR images.
% 
For instance, in the context of bird species classification, the task network may learn to utilize only beak features as a shortcut feature, rather than utilizing other essential bird features, such as wings or feet.
% 
In this scenario, employing such a task network as a TDP loss can limit the chance of SR to restore other essential bird features, which might be helpful for task performance.
% 
% Indeed, we observe that training the task network solely with HR images weakens the effectiveness of the TDP loss, which is analyzed in Section~\ref{}.


\begin{figure}[t!]
    \centering
    \subfloat[HR]{\includegraphics[width=0.3\linewidth]{example-image-a}}
    \hspace{2mm}
    \subfloat[SR]{\includegraphics[width=0.3\linewidth]{example-image-b}}
    \hspace{2mm}
    \subfloat[CQMix]{\includegraphics[width=0.3\linewidth]{example-image-c}}
    \\
    \figspace
    \caption{
        %
        \textbf{Concept of CQMix.}
        %
    }
    \label{fig:cqmix}
    \figxspace
\end{figure}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/submission/3.1/overall/overview4.pdf}
    \\
    \figspace
    \caption{
        %
        \textbf{Overview of the proposed TaSR.}
        % 
    }
    \label{fig:main_figure}
    \figxspace
\end{figure*}


To address this issue, we introduce a novel data augmentation strategy called Cross-Quality Patch Mix~(CQMix) during training the task network.
% 
The CQMix is designed to enhance the effectiveness of the TDP loss by encouraging the task network to learn more generalizable features.
% 
In particular, the CQMix augments an input image by randomly choosing either HR or SR patches for each grid region, as shown in Figure~\ref{fig:cqmix}.
% 
By doing so, CQMix creates an image where high-frequency components are randomly erased at a patch level, effectively preventing the task network from learning shortcut features in HR images.
% 
Moreover, it's noteworthy that our CQMix can be generally applied to various vision tasks if HR and LR pairs exist, unlike other data augmentation strategies that are specialized for specific tasks, such as Mix-Up~\cite{zhang2017mixup} or CutMix~\cite{yun2019cutmix} for image classification.
% 
% Figure~\ref{} describes the CQMix method and its intuitive meanings.
% 


\subsection{Alternate Training Framework}\label{subsec:alternate}
To leverage the TDP loss to enhance task performance, the task network must be capable of extracting meaningful features from input images relevant to the task.
% 
However, utilizing the feature space of a frozen task network can present challenges, as the network is not originally trained to extract meaningful features from intermediate SR results, which continue to evolve during training, potentially diminishing the effectiveness of the TDP loss.
% 

To resolve this issue, we propose an alternate training framework as shown in Figure~\ref{fig:main_figure}, which enables us to employ the feature space of the task network~$f_{\boldsymbol{\theta}_{\text{Task}}}$ for our TDP loss, rather than using the additional frozen task network.
% 
In the alternate training framework, one training iteration comprises two training phases.
% 
In the first phase, we train only the task network with a task-specific loss, \eg, cross-entropy loss for image classification, while freezing the SR network.
% 
Specifically, we train the task network using three types of images, HR, SR, and augmented images using the proposed CQMix.
% 
Then, in the second phase, we train only the SR network with pixel-wise reconstruction loss and proposed TDP loss using the feature space of $f_{\boldsymbol{\theta}_{\text{Task}}}$, while freezing the $f_{\boldsymbol{\theta}_{\text{Task}}}$.
% 
By doing so, since the task network is kept training using the intermediate SR results.
% 




Finally, the objective of our (name) is defined as follows:
\begin{equation}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{Task}}} \:\: & \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} (\boldsymbol{I}_{\text{aug}}), \boldsymbol{y}), & \text{\textit{in} phase 1,}\\
        \min\limits_{\boldsymbol{\theta}_{\text{SR}}} \:\: & \mathcal{L}_{\text{recon}}(f_{\boldsymbol{\theta}_{\text{SR}}} (\boldsymbol{I}_{\text{LR}}), \boldsymbol{I}_{\text{HR}}) + \mathcal{L}_{\text{TDP}}, & \text{\textit{in} phase 2,}\\
    \end{aligned}
\end{equation}
where $\boldsymbol{I}_{\text{aug}}$ is the concatenation of $\boldsymbol{I}_{\text{SR}}$, $\boldsymbol{I}_{\text{HR}}$, and the augmented images by CQMix.




\iffalse
\subsection{Overview: Cyclic Training}

To achieve the goal of task-aware super-resolution, a key question arises: \textit{How can we leverage the HR images and the task network to prompt the SR network to learn task-specific knowledge?}
Our strategy to address this question involves a cyclic training framework, alternating the training between the SR and task networks.
Figure~\ref{} illustrates the overview of our cyclic training scheme.
In the first cycle, the SR network is trained to generate images beneficial for the task network.
In the second cycle, the task network learns task-specific knowledge that will be transferred to the SR network in the subsequent cycle.
We elaborate on the details of the cyclic training framework in the following subsections.
In section~\ref{subsec:percep}, we introduce task-driven perceptual loss in the first cycle to encourage the SR network to imitate the task-relevant features present in HR images.
In section~\ref{subsec:mixup}, we share our observation that a task network trained solely on HR images learns less transferable features for the SR network.
Based on the observation, we introduce Cross-Quality patch Mix technique in the second cycle that prevents the task network from focusing on shortcuts, thereby enhancing the transferability for the SR network.


\subsection{Cycle 1: Task-Driven Perceptual Loss}\label{subsec:percep}
Owing to the abundance of features within HR images, training the task network with HR images achieves substantially better task performance compared to training with LR images.
For task-aware super-resolution to succeed, the SR network should strive to emulate HR images, particularly focusing on incorporating the task-relevant features present in HR images.
To this end, inspired by the concept of perceptual loss~\cite{leon2015_texture,misc_perceptual}, we propose task-driven perceptual loss that promotes the generation of SR images that imitate task-relevant and perceptually pleasing features within the HR images learned by the task network.
Formally, we define the task-driven perceptual loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{percep}} = \frac{1}{B} \sum_{i=1}^{B} \lVert f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
where $B$ is the batch size and the superscript in each image notation indicates the index of images in a batch.


In cycle 1, we train the SR network using the task-driven perceptual loss and the reconstruction loss between SR and HR images:
\begin{equation}
    \mathcal{L}_{\text{cycle 1}} = \mathcal{L}_{\text{percep}} + \mathcal{L}_{\text{recon}},
\end{equation}
where $\mathcal{L}_{\text{recon}} = \frac{1}{B} \sum_{i=1}^{B} \lVert \boldsymbol{I}_\text{SR}^i - \boldsymbol{I}_\text{HR}^i \rVert_1$.



\subsection{Cycle 2: Cross-Quality Patch Mix}\label{subsec:mixup}
To enhance the effectiveness of the task-driven perceptual loss, it is crucial that the task network learns task-specific features embedded in the HR images in cycle 2.
An intuitive approach is to train the task network with HR images.
Yet, we observe that training solely with HR images offers limited performance gain from the task-driven perceptual loss.
Instead, we find that training the task network using both the HR and upscaled LR images produces more performance gain.
Our hypothesis regarding this phenomenon is that training solely with HR images leads to shortcut learning, utilizing only a subset of HR image features for training.
This, in turn, hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
Figure~\ref{} illustrates the conceptual description of our hypothesis.
For a detailed analysis of these observations, please refer to Section~\ref{}.

Based on our observation, we propose a novel data augmentation strategy called \textbf{C}ross-\textbf{Q}uality patch \textbf{Mix} (CQMix) that further enhances the efficacy of the task-driven perceptual loss by encouraging the task network to learn more transferable knowledge for the SR network.
CQMix augments an image by randomly choosing either HR or SR patches within each grid region.
By doing so, CQMix creates an image where high-frequency components are randomly erased, effectively preventing the task network from learning shortcuts that are not transferable to the SR network.
Figure~\ref{} illustrates CQMix method and its intuitive meanings.
% 그래서 task net이 hr의 특정 feature에만 집중해서 학습하는걸 막고 다양한 feature를 학습하도록 강제함
%

Consequently, we train the task network in cycle 2 using task-specific loss using SR, HR, and augmented images by CQMix:
\begin{equation}
    \min\limits_{\boldsymbol{\theta}_\text{Task}} \; \sum_{i=1}^B \mathcal{L}_{\text{task}}(f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}^i),\boldsymbol{y}),
\end{equation}

\fi

\ifflase
\subsection{Alternate Training}\label{subsec:alternate}
In task-aware super-resolution problems, both the SR and task network keep changing throughout the training process.
In this circumstance, a possible approach to implement the task-driven perceptual loss is to incorporate an extra task network that is pre-trained on HR images.
However, due to the domain gap between the SR and HR images, the task network, exclusively trained on HR images, struggles to generate meaningful features of the SR images, undermining the effectiveness of the task-driven perceptual loss.
To resolve this issue, we propose an alternate training framework that enables the effective employment of task-driven perceptual loss when both the SR and task network change during training.
In the alternate training framework, one training iteration comprises two training phases.
In the first phase, we train only the task network with a task-specific loss using SR and HR images augmented by the CQMix method.
Then, in the second phase, we calculate the task-driven perceptual loss using the frozen task network.
Alongside the pixel-level reconstruction loss calculated between SR and HR images, the task-driven perceptual loss is employed for updating the SR network.

Finally, the objective of our (name) is defined as follows:
\begin{equation}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{Task}}} \:\: & \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} (\boldsymbol{I}_{\text{aug}}), \boldsymbol{y}), & \text{in phase 1,}\\
        \min\limits_{\boldsymbol{\theta}_{\text{SR}}} \:\: & \mathcal{L}_{\text{recon}}(f_{\boldsymbol{\theta}_{\text{SR}}} (\boldsymbol{I}_{\text{LR}}), \boldsymbol{I}_{\text{HR}}) + \mathcal{L}_{\text{percep}}, & \text{in phase 2,}\\
    \end{aligned}
\end{equation}
where $\boldsymbol{I}_{\text{aug}}$ is the concatenation of $\boldsymbol{I}_{\text{SR}}$, $\boldsymbol{I}_{\text{HR}}$, and the augmented images by CQMix.
The overview of (name) is illustrated in Figure~\ref{fig:main_figure}.
\fi


%%%%%%%%% proposed_method_v1.tex %%%%%%%%%%
\section{Proposed method}
\label{sec:proposed_method}
%
% Training the task network on HR images can achieve significantly superior results compared to training on their LR counterparts.
% % 
% This distinction is because LR images lack essential high-frequency details, which often contain crucial task-related features.
% 
% Therefore, to succeed in task-aware super-resolution, the SR network should prioritize restoring high-frequency regions, with a specific emphasis on the task-relevant features present in HR images.
% 
\paragraph{Overview.} 
% 
Our objective is to introduce a Task-aware Super-Resolution (TaSR) framework in which the SR network prioritizes the restoration of high-frequency regions relevant to specific tasks, consequently enhancing the performance of downstream tasks, such as image classification, semantic segmentation, and object detection.
% 

Figure~\ref{fig:overview} shows an overview of our method.
% 
Our approach involves two distinct training phases.
%
During the first phase, we exclusively train the SR network while keeping the task network frozen, using the TDP loss, as detailed in Section~\ref{subsec:percep}.
%
In the second phase, we exclusively train the task network while keeping the SR network frozen, employing our CQMix strategy, which will be elaborated upon in Section~\ref{subsec:mix}.
%
Lastly, we will delve into the benefits of the alternate training framework and introduce the training loss for each phase in Section~\ref{subsec:alternate}.
% 


\paragraph{Notation.}
Let $\boldsymbol{I}_\text{HR} \in \mathbb{I}_\text{HR}$ and $\boldsymbol{I}_\text{LR} \in \mathbb{I}_\text{LR}$ denote the high-resolution (HR) and low-resolution (LR) images, paired with their corresponding task labels $\boldsymbol{y} \in \mathbb{Y}$ (\eg, class labels in image classification task).
$f_{\boldsymbol{\theta}_{\text{SR}}}: \mathbb{I}_\text{LR} \rightarrow \mathbb{I}_\text{SR}$ denotes the super-resolution (SR) network parameterized by $\boldsymbol{\theta}_{\text{SR}}$ where $\mathbb{I}_\text{SR}$ is the super-resolved image set.
Given the SR images~$\boldsymbol{I}_\text{SR}$, we predict corresponding labels using the task network parameterized by $\boldsymbol{\theta}_{\text{Task}}$: $f_{\boldsymbol{\theta}_{\text{Task}}}: \mathbb{I}_\text{SR} \rightarrow \mathbb{Y}$.

\paragraph{Problem Definition.}
The goal of task-aware super-resolution is to produce photo-realistic images from $\boldsymbol{I}_\text{LR}$ that can benefit the subsequent high-level vision task, which is formally given by:
\begin{equation}\label{eq:problem_definition}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{SR}},\boldsymbol{\theta}_{\text{Task}}} & \mathcal{L}_{\text{SR}}(f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{I}_\text{HR}) \\ & + \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} \circ f_{\boldsymbol{\theta}_{\text{SR}}}(\boldsymbol{I}_\text{LR}),\boldsymbol{y}),
    \end{aligned}
\end{equation}
where the first and second terms are used to evaluate the quality of the super-resolved results and the performance for the target high-level vision task, respectively.

\subsection{Task-Driven Perceptual Loss}\label{subsec:percep}
% mse < percep : sr 측면에서
% 우리는 percep loss를 sr quality를 높이는거 + task에 도움이 되는 feature 집중해서 살리기 위해서
%
\iffalse
High-resolution (HR) images contain abundant high-frequency details crucial for achieving superior performance in high-level vision tasks, compared to low-resolution (LR) images.
Perceptual loss~\cite{leon2015_texture,misc_perceptual} is a widely used technique in the SR field to restore the high-frequency components present in HR images.
Conventionally, the perceptual loss is often calculated within a feature space of VGG network pre-trained on ImageNet, which might be irrelevant to a target task.
In the context of the task-aware super-resolution problem, however, it is essential for the SR network to strive to emulate HR images, particularly focusing on features relevant to a target task.
To this end, we propose task-driven perceptual loss, a more flexible usage of perceptual loss, that is calculated using the network trained on a target task.
By doing so, our task-driven perceptual loss can promote the generation of SR images that imitate not just visually appealing but also task-relevant high-frequency details contained in the HR images.
Formally, we define the task-driven perceptual loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{percep}} = \frac{1}{B} \sum_{i=1}^{B} \lVert f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
where $B$ is the batch size, and the superscript in each image notation indicates the index of images in a batch.
\fi

Perceptual loss~\cite{leon2015_texture, misc_perceptual} is a widely adopted technique in the field of SR to restore the high-frequency components.
% 
In particular, the perceptual loss is calculated as the distance between SR and HR images in the deep feature space, such as the VGG network pre-trained on ImageNet.
% 

In the perceptual loss,


As the perceptual loss quantifies the difference between SR and HR images in the feature space, the definition of this feature space significantly impacts the function of perceptual loss.
% 
Conventionally, the perceptual loss is computed within the feature space of a VGG network pre-trained on ImageNet.
% 
However, this feature space may not be directly relevant to the target task, and simply employing perceptual loss for updating ${\theta}_\text{SR}$ does not contribute to improving the performance of the subsequent task network $f_{\boldsymbol{\theta}_\text{Task}}$.
%


To this end, we propose task-driven perceptual~(TDP) loss, which offers a more flexible usage of perceptual loss by calculating the distance using the feature space of the task network, which is trained on a target task.
% 
When input images are fed into the task network, the deep neural network manipulates image features in a manner that enhances task execution.
% 
Hence, by computing the perceptual loss within the feature space of the task network, we can directly guide the SR network to restore high-frequency regions that are pertinent to the task.
% 
The TDP loss encourages the generation of SR images that not only appear visually appealing but also contain task-relevant high-frequency details.
% 
Formally, we define the TDP loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
% 
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{TDP}} = \frac{1}{B} \sum_{i=1}^{B} \lVert \phi_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - \phi_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
% 
where $B$ is the batch size, $\phi$ is an intermediate activation of the task network $f$, and the superscript in each image notation indicates the index of images in a batch.
% 


%In the following subsections, we introduce novel techniques to further enhance the effectiveness of our task-driven perceptual loss.
%In Section~\ref{subsec:mix}, we propose a novel data augmentation technique tailored for the task-aware super-resolution problem.
%In Section~\ref{subsec:alternate}, we propose an alternate training scheme that enables more gentle usage of the task-driven perceptual loss.


% 우리의 목표는 sr task 둘다 학습시키는 것
% 따라서 task network는 학습이 진행됨에 따라 계속 변함
% 이 상황에서 task percep을 줄 수 있는 방법은 additional pre-trained model 두는 것
% 하지만 이럴경우 
% 따라서 우리는 ~ 하기 위해 alterate training framework을 제안
% cycle 1 에서는~
% cycle 2 에서는~


\begin{figure}[t!]
    \centering
    \subfloat[HR]{\includegraphics[width=0.3\linewidth]{example-image-a}}
    \hspace{2mm}
    \subfloat[SR]{\includegraphics[width=0.3\linewidth]{example-image-b}}
    \hspace{2mm}
    \subfloat[CQMix]{\includegraphics[width=0.3\linewidth]{example-image-c}}
    \\
    \figspace
    \caption{
        %
        \textbf{Concept of CQMix.}
        %
    }
    \label{fig:cqmix}
    \figxspace
\end{figure}


\subsection{Cross-Quality Patch Mix}\label{subsec:mix}
\iffalse
The effectiveness of the task-driven perceptual loss is inherently related to the training procedure for the task network.
For high-level vision tasks, it is widely known that a network is susceptible to shortcut learning~\cite{geirhos2020shortcut}, which means a network relies on superficial and non-intrinsic features in training data, leading to poor generalization ability.
%cite classification suffer shortcut learning
% this could make the task-percep loss less effective since utilizing only a subset of HR image features hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
%We hypothesize that training solely with HR images leads to shortcut learning, utilizing only a subset of HR image features for training.
%This, in turn, hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
%Figure~\ref{} illustrates the conceptual description of our hypothesis.
Notably, shortcut learning can pose challenges in the problem of task-aware super-resolution, as the shortcut features learned by a task network can hinder the SR network from acquiring comprehensive features present in HR images through task-driven perceptual loss.
For instance, if a task network exclusively learns beak features to classify bird species, the task-driven perceptual loss may struggle to effectively guide the SR images to restore other key high-frequency contents, such as the feather and shape, limiting both the quality of SR results and the task performance.
Indeed, we observe that training the task network solely with HR images weakens the effectiveness of the task-driven perceptual loss, which is analyzed in Section~\ref{}.
\fi

Since our TDP loss operates within the feature space of the task network, its effectiveness is inherently linked to the training process of the task network.
% 
One possible approach is to utilize the feature space of a frozen task network pre-trained on HR images, similar to the conventional perceptual loss.
% 
However, it's crucial to recognize that task networks are susceptible to shortcut learning~\cite{geirhos2020shortcut}, a phenomenon where a network relies on superficial and non-intrinsic features in the training data.
% 
Notably, when we use a TDP loss using the task network trained with such shortcut learning, it can pose challenges, as it may hinder the SR network from acquiring the comprehensive features present in HR images.
% 
For instance, in the context of bird species classification, the task network may learn to utilize only beak features as a shortcut feature, rather than utilizing other essential bird features, such as wings or feet.
% 
In this scenario, employing such a task network as a TDP loss can limit the chance of SR to restore other essential bird features, which might be helpful for task performance.
% 
% Indeed, we observe that training the task network solely with HR images weakens the effectiveness of the TDP loss, which is analyzed in Section~\ref{}.


To address this issue, we introduce a novel data augmentation strategy called Cross-Quality Patch Mix~(CQMix) during training the task network.
% 
The CQMix is designed to enhance the effectiveness of the TDP loss by encouraging the task network to learn more generalizable features.
% 
In particular, the CQMix augments an input image by randomly choosing either HR or SR patches for each grid region, as shown in Figure~\ref{fig:cqmix}.
% 
By doing so, CQMix creates an image where high-frequency components are randomly erased at a patch level, effectively preventing the task network from learning shortcut features in HR images.
% 
Moreover, it's noteworthy that our CQMix can be generally applied to various vision tasks if HR and LR pairs exist, unlike other data augmentation strategies that are specialized for specific tasks, such as Mix-Up~\cite{zhang2017mixup} or CutMix~\cite{yun2019cutmix} for image classification.
% 
% Figure~\ref{} describes the CQMix method and its intuitive meanings.
% 



\subsection{Alternate Training Framework}\label{subsec:alternate}
To leverage the TDP loss to enhance task performance, the task network must be capable of extracting meaningful features from input images relevant to the task.
% 
However, utilizing the feature space of a frozen task network can present challenges, as the network is not originally trained to extract meaningful features from intermediate SR results, which continue to evolve during training, potentially diminishing the effectiveness of the TDP loss.
% 

To resolve this issue, we propose an alternate training framework as shown in Figure~\ref{fig:main_figure}, which enables us to employ the feature space of the task network~$f_{\boldsymbol{\theta}_{\text{Task}}}$ for our TDP loss, rather than using the additional frozen task network.
% 
In the alternate training framework, one training iteration comprises two training phases.
% 
In the first phase, we train only the task network with a task-specific loss, \eg, cross-entropy loss for image classification, while freezing the SR network.
% 
Specifically, we train the task network using three types of images, HR, SR, and augmented images using the proposed CQMix.
% 
Then, in the second phase, we train only the SR network with pixel-wise reconstruction loss and proposed TDP loss using the feature space of $f_{\boldsymbol{\theta}_{\text{Task}}}$, while freezing the $f_{\boldsymbol{\theta}_{\text{Task}}}$.
% 
By doing so, since the task network is kept training using the intermediate SR results.
% 

Finally, the objective of our (name) is defined as follows:
\begin{equation}
    \begin{aligned}
        \min\limits_{\boldsymbol{\theta}_{\text{Task}}} \:\: & \mathcal{L}_{\text{Task}}(f_{\boldsymbol{\theta}_{\text{Task}}} (\boldsymbol{I}_{\text{aug}}), \boldsymbol{y}), & \text{\textit{in} phase 1,}\\
        \min\limits_{\boldsymbol{\theta}_{\text{SR}}} \:\: & \mathcal{L}_{\text{recon}}(f_{\boldsymbol{\theta}_{\text{SR}}} (\boldsymbol{I}_{\text{LR}}), \boldsymbol{I}_{\text{HR}}) + \mathcal{L}_{\text{TDP}}, & \text{\textit{in} phase 2,}\\
    \end{aligned}
\end{equation}
where $\boldsymbol{I}_{\text{aug}}$ is the concatenation of $\boldsymbol{I}_{\text{SR}}$, $\boldsymbol{I}_{\text{HR}}$, and the augmented images by CQMix.




\iffalse
\subsection{Overview: Cyclic Training}

To achieve the goal of task-aware super-resolution, a key question arises: \textit{How can we leverage the HR images and the task network to prompt the SR network to learn task-specific knowledge?}
Our strategy to address this question involves a cyclic training framework, alternating the training between the SR and task networks.
Figure~\ref{} illustrates the overview of our cyclic training scheme.
In the first cycle, the SR network is trained to generate images beneficial for the task network.
In the second cycle, the task network learns task-specific knowledge that will be transferred to the SR network in the subsequent cycle.
We elaborate on the details of the cyclic training framework in the following subsections.
In section~\ref{subsec:percep}, we introduce task-driven perceptual loss in the first cycle to encourage the SR network to imitate the task-relevant features present in HR images.
In section~\ref{subsec:mixup}, we share our observation that a task network trained solely on HR images learns less transferable features for the SR network.
Based on the observation, we introduce Cross-Quality patch Mix technique in the second cycle that prevents the task network from focusing on shortcuts, thereby enhancing the transferability for the SR network.


\subsection{Cycle 1: Task-Driven Perceptual Loss}\label{subsec:percep}
Owing to the abundance of features within HR images, training the task network with HR images achieves substantially better task performance compared to training with LR images.
For task-aware super-resolution to succeed, the SR network should strive to emulate HR images, particularly focusing on incorporating the task-relevant features present in HR images.
To this end, inspired by the concept of perceptual loss~\cite{leon2015_texture,misc_perceptual}, we propose task-driven perceptual loss that promotes the generation of SR images that imitate task-relevant and perceptually pleasing features within the HR images learned by the task network.
Formally, we define the task-driven perceptual loss as the $\ell_1$ distance between the SR and HR images in the feature space of the task network:
\begin{equation}\label{eq:percep}
    \mathcal{L}_{\text{percep}} = \frac{1}{B} \sum_{i=1}^{B} \lVert f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{SR}^i) - f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}_\text{HR}^i) \rVert_1,
\end{equation}
where $B$ is the batch size and the superscript in each image notation indicates the index of images in a batch.


In cycle 1, we train the SR network using the task-driven perceptual loss and the reconstruction loss between SR and HR images:
\begin{equation}
    \mathcal{L}_{\text{cycle 1}} = \mathcal{L}_{\text{percep}} + \mathcal{L}_{\text{recon}},
\end{equation}
where $\mathcal{L}_{\text{recon}} = \frac{1}{B} \sum_{i=1}^{B} \lVert \boldsymbol{I}_\text{SR}^i - \boldsymbol{I}_\text{HR}^i \rVert_1$.



\subsection{Cycle 2: Cross-Quality Patch Mix}\label{subsec:mixup}
To enhance the effectiveness of the task-driven perceptual loss, it is crucial that the task network learns task-specific features embedded in the HR images in cycle 2.
An intuitive approach is to train the task network with HR images.
Yet, we observe that training solely with HR images offers limited performance gain from the task-driven perceptual loss.
Instead, we find that training the task network using both the HR and upscaled LR images produces more performance gain.
Our hypothesis regarding this phenomenon is that training solely with HR images leads to shortcut learning, utilizing only a subset of HR image features for training.
This, in turn, hinders the SR network from acquiring comprehensive features present in HR images through the task-driven perceptual loss.
Figure~\ref{} illustrates the conceptual description of our hypothesis.
For a detailed analysis of these observations, please refer to Section~\ref{}.

Based on our observation, we propose a novel data augmentation strategy called \textbf{C}ross-\textbf{Q}uality patch \textbf{Mix} (CQMix) that further enhances the efficacy of the task-driven perceptual loss by encouraging the task network to learn more transferable knowledge for the SR network.
CQMix augments an image by randomly choosing either HR or SR patches within each grid region.
By doing so, CQMix creates an image where high-frequency components are randomly erased, effectively preventing the task network from learning shortcuts that are not transferable to the SR network.
Figure~\ref{} illustrates CQMix method and its intuitive meanings.
% 그래서 task net이 hr의 특정 feature에만 집중해서 학습하는걸 막고 다양한 feature를 학습하도록 강제함
%

Consequently, we train the task network in cycle 2 using task-specific loss using SR, HR, and augmented images by CQMix:
\begin{equation}
    \min\limits_{\boldsymbol{\theta}_\text{Task}} \; \sum_{i=1}^B \mathcal{L}_{\text{task}}(f_{\boldsymbol{\theta}_\text{Task}}(\boldsymbol{I}^i),\boldsymbol{y}),
\end{equation}

\fi


%%%%%%%%% Introduction_v0.tex %%%%%%%%%%

%%%%%%%%% Introduction_v0.tex %%%%%%%%%%


==> tables/submission/4.2/ablation/ablation.tex <==
\begin{table*}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{C{2.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}}
\specialrule{.1em}{.05em}{.05em}
\hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Accuracy} & \multicolumn{3}{c}{Complexity}\\
\cline{2-6}
& PSNR & SSIM & MACs & VRAM & Params\\
\specialrule{.1em}{.05em}{.05em}
ClassConv & 30.77 & 0.9105 & 13.79 & & 8.93 \\
\hline
$\text{ClassConv}^{ran}$ & 30.50 & 0.9060 & 13.79 & & 8.93\\
$\text{ClassConv}^{all}$ & 30.51 & 0.9062 & 39.66 & & 8.93\\
$\text{ClassConv}^{gt}$ & 30.86 & 0.9117 & 13.79 & & 8.93\\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}
\caption{
    \textbf{Ablation studies on ClassConv.} 
    sample.
}
\label{table:parameter}
\end{table*}

==> tables/submission/4.2/annealing/annealing.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{L{4.0cm}C{1.3cm}C{1.3cm}}
% % \specialrule{.1em}{.05em}{.05em}
% \toprule
% \,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro}\\
% % \cline{2-3}
% & PSNR & SSIM\\
% \hline
% \;~U-Net & 30.43 & 0.9049 \\
% \;~+~\textbf{B-conv} & 30.67 & 0.9081 \\
% \;~+~\textbf{B-conv} \emph{without} annealing. & 30.53 & 0.9055 \\
% % \hline
% \bottomrule
% \end{tabular}
% \caption{
%     \textbf{Effect of annealing strategy.}
%     %
%     Without an annealing strategy, performance boosting from B-conv largely decreases.
%     % 
% }
% \label{table:effect_of_annealing}
% \end{table}

% % \begin{table}
% % \small
% % \centering
% % \setlength\tabcolsep{1.0pt}
% % \def\arraystretch{1.1}
% % \begin{tabular}{L{5.0cm}|C{1.3cm}|C{1.3cm}}
% % % \specialrule{.1em}{.05em}{.05em}
% % \toprule
% % % \hline
% % \multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro}\\
% % \cline{2-3}
% % & PSNR & SSIM\\
% % % \hline
% % \hline
% % \textbf{B-conv} & 30.67 & 0.9081 \\
% % \textbf{B-conv} \emph{without} annealing. & 30.53 & 0.9055 \\
% % % \hline
% % \bottomrule
% % \end{tabular}
% % \caption{
% %     \textbf{Effect of annealing strategy.}
% %     %
% %     Without an annealing strategy, performance boosting from B-conv largely decreases.
% %     % 
% % }
% % \label{table:effect_of_annealing}
% % \end{table}

==> tables/submission/4.2/annealing_pixelwise/annealing_pixelwise.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{L{3.0cm}|C{1.3cm}|C{1.3cm}|C{2.0cm}}
% % \specialrule{.1em}{.05em}{.05em}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{GoPro} & \multicolumn{1}{c}{Complexity}\\
% \cline{2-4}
% & PSNR & SSIM & Params\\
% \hline
% % \hline
% Pixel-wise~(\textbf{S-conv}) & 30.67 & 0.9081 & (0.09) + 6.82  \\
% Patch-wise & 30.20 & 0.8996 & (0.09) + 7.85  \\
% % \specialrule{.1em}{.05em}{.05em}
% \bottomrule
% \end{tabular}
% \caption{
%     \textbf{Advantage of the pixel-wise operation.}
%     %
% }
% \label{table:advantage_from_pixelwise}
% \end{table}


% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{2.6cm}|C{1.0cm}|C{1.0cm}|C{1.6cm}|C{1.6cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{GoPro} & \multicolumn{2}{c}{Complexity}\\
% \cline{2-5}
% & PSNR & SSIM & MACs & Params\\
% \hline
% \hline
% Pixel-wise~(\textbf{S-conv}) & 30.67 & 0.9081 & (0.09) + 6.82  \\
% Patch-wise & 30.20 & 0.8996 & (0.09) + 7.85  \\
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \end{tabular}
% \caption{
%     \textbf{Advantage from pixel-wise operation.}
%     %
%     The number in parenthesis is from blur level regression network $\mathcal{R}$.
%     %
% }
% \label{table:baseline_performance}
% \end{table}


\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{4.5cm}C{1.3cm}C{1.3cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro} \\
& PSNR & SSIM \\
\hline
\;~U-Net & 30.43 & 0.9049 \\
\;~+~\textbf{B-conv} & 30.67 & 0.9081 \\
\;~+~\textbf{B-conv} \emph{without} annealing. & 30.53 & 0.9055 \\
% \specialrule{.1em}{.05em}{.05em}
\bottomrule
\end{tabular}
\caption{
    \textbf{Effect of annealing strategy and pixel-wise operation.}
    %
    The performance boosting of B-conv largely decreases when the annealing strategy is not adopted, demonstrating its effectiveness.
    % 
}
\label{table:annealing_pixelwise}
\end{table}

==> tables/submission/4.2/baseline/baseline.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{2.5cm}|C{1.3cm}|C{1.3cm}|C{2.0cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% Methods & PSNR & SSIM & MACs \\
% \specialrule{.1em}{.05em}{.05em}
% Baseline & 30.43 & 0.9050 & 13.79 \\
% % Baseline$^\text{chan+}$ & 30.46 & 0.9053 & 14.64 \\
% % \hline
% ClassConv & 30.67 & 0.9085 & (0.52) + 13.79 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Performance of the proposed ClassConv.} 
%     sample.
% }
% \label{table:baseline}
% \end{table}

\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{2.2cm}C{1.1cm}C{1.1cm}C{1.6cm}C{1.6cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro} & \multirow{2}{*}{MACs~(G)} & \multirow{2}{*}{Latency~(s)} \\
& PSNR & SSIM & &\\
\hline
% \;~U-Net & 30.43 & 0.9049 & 13.79 & 2.61 \\
% \;~+~\textbf{B-conv} & 30.67 & 0.9081 & +~0.52 & +~4.30 \\
% % Conv (+chan) & 30.46 & 0.9053 & 14.64 & & 2.78 \\
% \hline
% \;~Baseline~\cite{db_nafnet} & 32.24 & 0.9311 & 15.96 & 17.0\\
% \;~+~\textbf{B-conv} & 32.34 & 0.9321 & +~0.52 & +25.9\\
% \hline
% \;~NAFNet~\cite{db_nafnet} & 32.31 & 0.9321 & 12.29 & 12.1\\
% \;~+~\textbf{B-conv} & 32.36 & 0.9326 & +~0.52 & + 17.6\\

\;~U-Net & 30.43 & 0.9049 & 13.79 & 0.265 \\
\;~+~\textbf{B-conv} & 30.67 & 0.9081 & 14.31 & 0.333 \\
% Conv (+chan) & 30.46 & 0.9053 & 14.64 & & 2.78 \\
\hline
\;~Baseline~\cite{db_nafnet} & 32.24 & 0.9311 & 15.96 & 0.284 \\
\;~+~\textbf{B-conv} & 32.34 & 0.9321 & 16.48 & 0.362 \\
\hline
\;~NAFNet~\cite{db_nafnet} & 32.31 & 0.9321 & 12.29 & 0.231 \\
\;~+~\textbf{B-conv} & 32.36 & 0.9326 & 12.81 & 0.287 \\

\bottomrule
\end{tabular}
\caption{
    \textbf{Advantage of applying B-conv to various deblurring architectures.}
    %
    % The proposed B-conv significantly boosts the performance of the U-Net, with only negligible increment on computatonal cost~($\sim$4\%).
    % The MACs~(G) is calculated from the patch with 256$\times$256 size, VRAM~(MB) is measured in a single RTX 2080 TI, and the number of parameters is in million~(M) units.
    %
    MACs and Latency are calculated for a $256 \times 256$ input.
    % 
    We note that the additional latency caused by the blur level predictor is about 0.026s.
}
\label{table:baseline_performance}
\end{table}


% \begin{table}
% \small
% \newcommand{\spacing}{\;}
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{L{3.9cm}C{1.1cm}C{1.1cm}C{1.7cm}}
% % \specialrule{.1em}{.05em}{.05em}
% \toprule{}
% % \hline
% \multirow{2}{*}{\,Methods} & \multicolumn{2}{c}{GoPro} & \multirow{2}{*}{MACs~(G)}\\
% % \cline{2-4}
% & PSNR & SSIM & \\
% \hline
% % \hline
% % Baseline-width32~\cite{db_nafnet} & 31.69 & 0.9247 & 15.96 \\
% % Baseline-width32~\cite{db_nafnet} +~S-conv & 31.75 & 0.9250 & (0.52) + 15.96 \\
% \spacing~Baseline$^\text{\ding{61}}$\cite{db_nafnet} & 32.24 & 0.9311 & 15.96 \\
% \spacing~+~\textbf{B-conv} & 32.34 & 0.9321 & +~0.52 \\
% \hline
% % NAFNet-width32~\cite{db_nafnet} & 31.69 & 0.9248 & 12.29 \\
% % NAFNet-width32~\cite{db_nafnet} +~S-conv & 31.76 & 0.9254 & (0.52) + 12.29 \\
% \spacing~NAFNet~\cite{db_nafnet} & 32.31 & 0.9321 & 12.29 \\
% \spacing~+~\textbf{B-conv} & 32.36 & 0.9326 & +~0.52 \\
% % \hline
% % \specialrule{.1em}{.05em}{.05em}
% \bottomrule
% \end{tabular}
% \caption{
%     \textbf{Application on state-of-the-art networks.}
%     %
%     We put notation~(\ding{61}) to avoid confusion with our baseline network.
%     %
% }
% \label{table:performance_boosting}
% \end{table}

==> tables/submission/4.2/importance_blur_level/importance_blur_level.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{5.0cm}C{1.3cm}C{1.3cm}}
\toprule
\,~\multirow{2}{*}{Policy for input map $\hat{\mathcal{B}}$} & \multicolumn{2}{c}{GoPro}\\
& PSNR & SSIM\\
\hline
\;~Random & 30.39 & 0.9044 \\
\;~Restoration difficulty & 30.45 & 0.9052 \\
\;~\textbf{Blur level}~(Estimated, patch-wise) & 30.52 & 0.9063 \\
\;~\textbf{Blur level}~(Estimated) & 30.67 & 0.9081 \\
\hline
\;~\textbf{Blur level}~(Ground-truth) & 30.73 & 0.9091 \\
\bottomrule
\end{tabular}
\caption{
    \textbf{Importance of blur level in our B-conv.}
    %
    % Employing blur level as labeling strategy performs the best, demonstrating the importance of blur level when handling dynamic scenes.
    %We note that the map from each labeling map policy is used as input for our B-conv.
    We note that U-Net without B-conv achieves 30.43dB PSNR on the GoPro dataset.
    %
    For random and ground-truth policies, we use predetermined input maps $\mathcal{B}$ following the policy instead of an output of the predictor.
}
\label{table:importance_blur_level}
\end{table}

% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{L{4.4cm}C{1.6cm}C{1.6cm}}
% \toprule
% \,~\multirow{2}{*}{Labeling strategy} & \multicolumn{2}{c}{GoPro}\\
% & PSNR & SSIM\\
% \hline
% \;~Random label & 30.39 & 0.9044 \\
% \;~Restoration difficulty & 30.45 & 0.9052 \\
% \;~Estimated blur level~(\textbf{B-conv}) & 30.67 & 0.9081 \\
% \hline
% \;~Ground-truth blur level & 30.73 & 0.9091 \\
% \bottomrule
% \end{tabular}
% \caption{
%     \textbf{Importance of blur level.}
%     %
%     Adopting blur level as labeling strategy performs the best, demonstrating the importance of blur level when handling dynamic scenes.
%     % 
% }
% \label{table:importance_blur_level}
% \end{table}


% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{L{4.4cm}|C{1.6cm}|C{1.6cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \,~\multirow{2}{*}{Labeling strategy} & \multicolumn{2}{c}{GoPro}\\
% \cline{2-3}
% & PSNR & SSIM\\
% \hline
% \hline
% \;~Random label & 30.39 & 0.9044 \\
% \;~Restoration difficulty & 30.45 & 0.9052 \\
% \;~Estimated blur level~(\textbf{B-conv}) & 30.67 & 0.9081 \\
% \hline
% \;~Ground-truth blur level & 30.73 & 0.9091 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Importance of blur level.}
%     %
%     Adopting blur level as labeling strategy performs the best, demonstrating the importance of blur level when handling dynamic scenes.
%     % 
% }
% \label{table:importance_blur_level}
% \end{table}

==> tables/submission/4.3/analysis_improvement/analysis_improvement.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{3.6cm}C{1.4cm}C{1.4cm}C{1.4cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{3}{c}{PSNR on GoPro}\\
& Level~1 & Level~2 & Level~3 \\
\hline
\;~U-Net & 33.21 & 30.71 & 28.86 \\
\;~+~\textbf{B-conv} & 33.55 & 30.90 & 28.82 \\
\hline
\;~+~\textbf{B-conv}~$\paren{\mathcal{B} = 1}$ & \textbf{33.54} & 29.03 & 24.89 \\
\;~+~\textbf{B-conv}~$\paren{\mathcal{B} = 2}$ & 31.93 & \textbf{30.87} & 27.27 \\
\;~+~\textbf{B-conv}~$\paren{\mathcal{B} = 3}$ & 27.89 & 27.65 & \textbf{28.76} \\
\bottomrule
\end{tabular}
\caption{
    \textbf{Analysis on performance improvement from B-conv.}
    % 
    $\mathcal{B} = l$ denotes that the input blur level map $\mathcal{B}$ is not an output of the predictor, but a constant matrix where all of its elements are $l$.
    % 
}
\label{table:analysis_improvement}
\end{table}

==> tables/submission/4.3/application_sota/application_sota.tex <==
\begin{table}
\small
\newcommand{\spacing}{\;}
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{3.9cm}C{1.1cm}C{1.1cm}C{1.7cm}}
% \specialrule{.1em}{.05em}{.05em}
\toprule{}
% \hline
\multirow{2}{*}{\,Methods} & \multicolumn{2}{c}{GoPro} & \multirow{2}{*}{MACs~(G)}\\
% \cline{2-4}
& PSNR & SSIM & \\
\hline
% \hline
% Baseline-width32~\cite{db_nafnet} & 31.69 & 0.9247 & 15.96 \\
% Baseline-width32~\cite{db_nafnet} +~S-conv & 31.75 & 0.9250 & (0.52) + 15.96 \\
\spacing~Baseline$^\text{\ding{61}}$\cite{db_nafnet} & 32.24 & 0.9311 & 15.96 \\
\spacing~+~\textbf{B-conv} & 32.34 & 0.9321 & +~0.52 \\
\hline
% NAFNet-width32~\cite{db_nafnet} & 31.69 & 0.9248 & 12.29 \\
% NAFNet-width32~\cite{db_nafnet} +~S-conv & 31.76 & 0.9254 & (0.52) + 12.29 \\
\spacing~NAFNet~\cite{db_nafnet} & 32.31 & 0.9321 & 12.29 \\
\spacing~+~\textbf{B-conv} & 32.36 & 0.9326 & +~0.52 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
\bottomrule
\end{tabular}
\caption{
    \textbf{Application on state-of-the-art networks.}
    %
    We put notation~(\ding{61}) to avoid confusion with our baseline network.
    %
}
\label{table:application_on_sota}
\end{table}

==> tables/submission/4.3/blur_regression/blur_regression.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{3.5cm}|C{1.8cm}|C{1.8cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c}{Accuracy}\\
% \cline{2-3}
% & GoPro & REDS\\
% \hline
% \hline
% Regression network~$\mathcal{R}$ & 84.96 \% & 90.77 \% \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Blur level regression accuracy.}
% }
% \label{table:blur_regression}
% \end{table}


\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{3.6cm}C{1.8cm}C{1.8cm}}
\toprule
\,~\multirow{2}{*}{} & \multicolumn{2}{c}{Accuracy}\\
& GoPro & REDS\\
\hline
\;~Blur level predictor~$\mathcal{P}$ & 84.96 \% & 90.77 \% \\
\bottomrule
\end{tabular}
\caption{
    \textbf{Blur level prediction accuracy.}
    % 
    % Even with the CNN-based network with small computational overhead, the prediction works sufficiently well on GoPro and REDS datasets.
    The accuracy is calculated with the number of blur levels $L=3$.
    % 
    % Our predictor introduces a small computational overhead with 0.52G MACs for $256\times256$ input.
}
\label{table:blur_level_accuracy}
\end{table}


==> tables/submission/4.3/number_level/number_level.tex <==
\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{2.6cm}C{1.1cm}C{1.1cm}C{1.4cm}C{1.7cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro} & \multirow{2}{*}{MACs~(G)} & \multirow{2}{*}{Latency~(s)}\\
& PSNR & SSIM & & \\
\hline
% \;~U-Net & 30.43 & 0.9049 & 13.79 & 2.61 \\
% \;~+~\textbf{B-conv}~$\paren{n = 2}$ & 30.62 & 0.9074 & +~0.52 & +~2.20  \\
% \;~+~\textbf{B-conv}~$\paren{n = 3}$ & 30.67 & 0.9081 & +~0.52 & +~4.30 \\
% \;~+~\textbf{B-conv}~$\paren{n = 4}$ & 30.69 & 0.9085 & +~0.52 & +~6.41 \\
\;~U-Net & 30.43 & 0.9049 & 13.79 & 0.265 \\
\;~+~\textbf{B-conv}~$\paren{L = 2}$ & 30.62 & 0.9074 & 14.31 & 0.328 \\
\;~+~\textbf{B-conv}~$\paren{L = 3}$ & 30.67 & 0.9081 & 14.31 & 0.333 \\
\;~+~\textbf{B-conv}~$\paren{L = 4}$ & 30.69 & 0.9085 & 14.31 & 0.337 \\
\bottomrule
\end{tabular}
\caption{
    \textbf{Effect of the number of blur levels.}
    %
    % The performance-boosting is further improved along with the number of blur levels increases. However, the improvement gap steadily decreases.
    MACs and Latency are calculated for a $256 \times 256$ input.
    % 
    We note that $L$ represents the number of the blur level used in our B-conv.
    % 
}
\label{table:number_level}
\end{table}


% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{2.5cm}|C{1.3cm}|C{1.3cm}|C{2.5cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{GoPro} & \multicolumn{1}{c}{Complexity}\\
% \cline{2-4}
% & PSNR & SSIM & Params\\
% \hline
% \hline
% $n = 2$ & 30.62 & 0.9074 & (0.09) + 4.72  \\
% $n = 3$ & 30.67 & 0.9081 & (0.09) + 6.82  \\
% $n = 4$ & 30.69 & 0.9085 & (0.09) + 8.93  \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Number of the blur level.}
%     %
% }
% \label{table:number_level}
% \end{table}


==> tables/submission/4.3/performance_reds/performance_reds.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{3.5cm}|C{1.3cm}|C{1.3cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{2}{c}{REDS}\\
% \cline{2-3}
% & PSNR & SSIM\\
% \hline
% \hline
% conv & 32.02 & 0.9026 \\
% \textbf{B-conv} & 32.24 & 0.9061 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Performance boosting of the B-conv in REDS dataset.}
%     %
% }
% \label{table:performance_reds}
% \end{table}

\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{3.6cm}C{1.8cm}C{1.8cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{REDS}\\
& PSNR & SSIM\\
\hline
\;~U-Net & 32.02 & 0.9026 \\
\;~+~\textbf{B-conv} & 32.24 & 0.9061 \\
\bottomrule
\end{tabular}
\caption{
    \textbf{Generalization of the B-conv on the REDS dataset.}
    %
    % The proposed B-conv consistently increases the performance also in the REDS~\cite{data_reds} dataset, demonstrating its scalability.
    %
}
\label{table:performance_reds}
\end{table}


==> tables/supple/baseline_corrected/baseline_corrected.tex <==
% \begin{table}
% \small
% \centering
% \setlength\tabcolsep{1.0pt}
% \def\arraystretch{1.1}
% \begin{tabular}{C{2.5cm}|C{1.3cm}|C{1.3cm}|C{2.0cm}}
% \specialrule{.1em}{.05em}{.05em}
% \hline
% Methods & PSNR & SSIM & MACs \\
% \specialrule{.1em}{.05em}{.05em}
% Baseline & 30.43 & 0.9050 & 13.79 \\
% % Baseline$^\text{chan+}$ & 30.46 & 0.9053 & 14.64 \\
% % \hline
% ClassConv & 30.67 & 0.9085 & (0.52) + 13.79 \\
% \hline
% \specialrule{.1em}{.05em}{.05em}
% \end{tabular}
% \caption{
%     \textbf{Performance of the proposed ClassConv.} 
%     sample.
% }
% \label{table:baseline}
% \end{table}

\begin{table}
\small
\centering
\setlength\tabcolsep{1.0pt}
\def\arraystretch{1.1}
\begin{tabular}{L{2.2cm}C{1.1cm}C{1.1cm}C{1.6cm}C{1.6cm}}
\toprule
\,~\multirow{2}{*}{Methods} & \multicolumn{2}{c}{GoPro} & \multirow{2}{*}{MACs~(G)} & \multirow{2}{*}{Latency~(s)} \\
& PSNR & SSIM & &\\
\hline
% \;~U-Net & 30.43 & 0.9049 & 13.79 & 2.61 \\
% \;~+~\textbf{B-conv} & 30.67 & 0.9081 & +~0.52 & +~4.30 \\
% % Conv (+chan) & 30.46 & 0.9053 & 14.64 & & 2.78 \\
% \hline
% \;~Baseline~\cite{db_nafnet} & 32.24 & 0.9311 & 15.96 & 17.0\\
% \;~+~\textbf{B-conv} & 32.34 & 0.9321 & +~0.52 & +25.9\\
% \hline
% \;~NAFNet~\cite{db_nafnet} & 32.31 & 0.9321 & 12.29 & 12.1\\
% \;~+~\textbf{B-conv} & 32.36 & 0.9326 & +~0.52 & + 17.6\\

\;~U-Net & 30.43 & 0.9049 & 13.79 & 0.265 \\
\;~+~\textbf{B-conv} & 30.67 & 0.9081 & 14.31 & 0.333 \\
% Conv (+chan) & 30.46 & 0.9053 & 14.64 & & 2.78 \\
\hline
\;~Baseline~\citenumber{2} & 32.24 & 0.9311 & 15.96 & 0.284 \\
\;~+~\textbf{B-conv} & 32.34 & 0.9321 & \textcolor{BrickRed}{16.48} & 0.362 \\
\hline
\;~NAFNet~\citenumber{2} & 32.31 & 0.9321 & 12.29 & 0.231 \\
\;~+~\textbf{B-conv} & 32.36 & 0.9326 & \textcolor{BrickRed}{12.81} & 0.287 \\

\bottomrule
\end{tabular}
\caption{
    \textbf{Advantage of applying B-conv to various deblurring architectures.}
    %
    We denote the corrected value as \textcolor{BrickRed}{\textbf{red}} color.
}
\label{table:baseline_performance_corrected}
\end{table}
